Persuading Voters in District-based Elections

We focus on the scenario in which an agent can exploit his information advantage to manipulate the outcome of an election. In particular, we study district-based elections with two candidates, in which the winner of the election is the candidate that wins in the majority of the districts. District-based elections are adopted worldwide (e.g., UK and USA) and are a natural extension of widely studied voting mechanisms (e.g., k-voting and plurality voting). We resort to the Bayesian persuasion framework, where the manipulator (sender) strategically discloses information to the voters (receivers) that update their beliefs rationally. We study both private signaling, in which the sender can use a private communication channel per receiver, and public signaling, in which the sender can use a single communication channel for all the receivers. Furthermore, for the first time, we introduce semi-public signaling in which the sender can use a single communication channel per district. We show that there is a sharp distinction between private and (semi-)public signaling. In particular, optimal private signaling schemes can provide an arbitrarily better probability of victory than (semi-)public ones and can be computed efficiently, while optimal (semi-)public signaling schemes cannot be approximated to within any factor in polynomial time unless P=NP. However, we show that reasonable relaxations allow the design of multi-criteria PTASs for optimal (semi-)public signaling schemes. In doing so, we introduce a novel property, namely comparative stability, and we design a bi-criteria PTAS for public signaling in general Bayesian persuasion problems beyond elections when the sender's utility function is state-dependent.

==> abstract.tex <==
\chapter*{\textbf{Abstract}}


Following the 2016 US presidential elections a number of commentators have suggested that Donald Trump would not have been elected president were it not for the influence of fake news.
%
As we approach the next presidential election, the question of how the spread of false and misleading news can affect the election result has gain renewed interest.
%

%
In this work, we model this problem by means of the Bayesian persuasion framework and ask whether it is computationally tractable to design a signaling scheme maximizing the probability with which a target candidate is elected in a district-based election.
%
Given the variety of possible media over which fake news can circulate, we analyse three different types of signaling schemes: private, public and the novelty concept of semi-public signaling scheme.
%

%
We show that the sender is not indifferent with respect to which kind of media is chosen to disclose fake news.
%
In particular, we prove that the sender can perform arbitrarily worse when restricted to use public or semi-public signaling schemes.
%

%
The different signaling schemes show a stark contrast also in terms of their computational complexity.
%
When private signals are allowed, we show that an optimal signaling scheme can be efficiently computed.
%
On the other hand, the sender’s optimal expected utility cannot be even approximated in polynomial time, using public or semi-public signaling schemes. 
%

%
In an attempt to overcome these inapproximability results, we introduce a new concept of stability, and we study the general problem of computing approximately optimal public signaling schemes when the sender's objective is replaced by another function, that approximates and is stable compared to the original objective.
%
In this context, we provide an important contribution by extending the previous results to the case of state-dependent objective functions.
%

%
Finally, we employ this result to provide efficient tri-criteria approximation algorithms for computing public and semi-public signaling schemes in district-based elections.

==> notation.tex <==
%\begin{tabular}{c|c}
%	\hline $k \in \K$ & types \\
%	\hline $\nType$  & num types \\
%	\hline $\A$ & actions of the receivers\\
%	\hline $\nAct$ & num action receiver\\
%	\hline $\theta \in \Theta$ & states of natures\\
%	\hline $\nState$ & num states\\
%	\hline $u_\theta^k(a)\in [0,1]$ & utility of type $k$ in state $\theta$ playing action $a$\\
%	\hline $u^s_\theta(a)\in [0,1]$ &utility of sender in state $\theta$ when receiver plays action $a$\\
%	\hline $\mu\in\textnormal{int}(\Delta_\Theta)$ & prior\\
%	\hline $\phi$& signaling scheme\\
%	\hline $s$& signal\\
%	\hline $\pvec$ & posterior\\
%	 \hline $W=\{(\pvec,w_\pvec)\}$ & signaling scheme as the weighted set of posteriors\\
%	 \hline $W(\phi)$& set $W$ induced by $\phi$\\
%	 \hline $\brset^k_\pvec$& best response set of type $k$ in posterior $\pvec$\\
%	 \hline $\best^k_p$ & best response of type $k$ in posterior $\pvec$ that maximizes the utility of the sender\\
%	 \hline $\brseteps^k_p$ & $\epsilon$ best response set of type $k$ in posterior $\pvec$\\
%	 \hline $\bestEps^k_p$ & $\epsilon$ best response of type $k$ in posterior $\pvec$ that maximizes the utility of the sender\\
%	 \hline $\kvec$ & sequence of types\\
%	 \hline $k^t$ & the $t$ element of the sequence\\
%	\hline $u^s(\phi,k)$ and $u^s(p,k)$ & expected utility of the sender with signaling scheme $\phi$(or posterior p) and type $k$\\
%	\hline $R^T$ &regret\\
%	\hline $R^T_\epsilon$ & regret signal $\epsilon$ persuasive\\
%	
%	
%\end{tabular}


\clearpage


\begin{tabular}{c|c}
	$R^d$ & receivers in district $d$\\
\hline
 	$\W$ & aggregate voting function\\
 	\hline
  W &internal voting function\\	
  \hline
  $\bar W$ & external voting funcion\\
  \hline
  $\cvec$ & action profile\\
  \hline
  $\cvec^d$ & action profile of voters in district d\\
  \hline
  $u_r(\theta)$ & utility in state $\theta$\\
  \hline
  $p \in P$ & posteriors\\
  \hline
  $\s \in \S$ & signals\\
  \hline
   $\s_r \in \S_r$ & signal of receiver $r$\\
  \hline
  $\phi \in \Phi$ & signaling schemes\\
  \hline
  $\phi_r(\theta,c) $& marginal signals\\
  

\end{tabular}
